Manipulation of oral cancer speech using neural articulatory synthesis

We present an articulatory synthesis framework for the synthesis and manipulation of oral cancer speech for clinical decision making and alleviation of patient stress. Objective and subjective evaluations demonstrate that the framework has acceptable naturalness and is worth further investigation. A subsequent subjective vowel and consonant identification experiment showed that the articulatory synthesis system can manipulate the articulatory trajectories so that the synthesised speech reproduces problems present in the ground truth oral cancer speech.

==> tables/full_table.tex <==

\begin{table*}
\caption{Objective evaluation of the naturalness results quantified by the MCD (in dB) for the SEEN and PSEEN experimental conditions. The columns contain the identifier and type of the speaker (control/oral cancer). The rows contain the value of the standard deviation parameter used during the data augmentation experiments. }
\begin{tabular}{l|cc|ccccc||cc|ccccc}
\toprule
 {} & \multicolumn{7}{|c||}{UNSEEN} & \multicolumn{7}{|c}{PSEEN} \\
 \midrule
 {} & \multicolumn{2}{|c|}{Control} & \multicolumn{5}{|c||}{Oral cancer} & \multicolumn{2}{|c|}{Control} & \multicolumn{5}{|c}{Oral cancer}\\
 \midrule
{} & 07hc & 01hc & 02pt &   03pt &   04pt & 05pt & 06pt & 07hc & 01hc & 02pt & 03pt & 04pt &  05pt &  06pt \\
\midrule
no noise &   7.48  &   7.59  &   7.09  &     8.38  &     6.65  &   7.79  &   7.34  &    8.7  &   7.91  &   8.16  &   8.89  &   7.17  &     8.32  &     8.5  \\
0.001    &   7.48  &   7.59  &   7.08  &     8.38  &     6.62  &   7.79  &   7.35  &    8.7  &   7.91  &   8.16  &   8.89  &   7.16  &     8.31  &     8.5  \\
0.01     &   7.41  &   7.57  &   7.08  &  8.06 (*) &     6.61  &   7.66  &   7.25  &   8.69  &   7.95  &   8.17  &   8.88  &   7.17  &     8.24  &    8.48  \\
0.1      &   7.36  &    7.5  &   7.05  &     8.46  &  6.58 (*) &   8.02  &    7.3  &   8.67  &   8.01  &   8.22  &   8.89  &   7.22  &  8.56 (*) &  8.7 (*) \\
\bottomrule

\end{tabular}

\end{table*}

==> tables/mos_table.tex <==
\begin{table}
\caption{MOS results of the naturalness experiment. (TODO: IN PROGRESS) }
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc|ccccc}
\toprule
 {} & \multicolumn{2}{|c|}{Control} & \multicolumn{5}{|c}{Oral cancer}  \\
 \midrule
{} & 07hc & 01hc & 02pt &   03pt &   04pt & 05pt & 06pt \\
\midrule
original    &     4.55 &     4.88 &     4.10 &     4.40 &     3.30 &     4.32 &     4.03 \\
resynthesis &     4.05 &     4.95 &     3.85 &     3.50 &     3.20 &     3.88 &     4.03 \\
predicted   &     1.88 &     2.55 &     2.25 &     1.85 &     2.17 &     2.48 &     1.88 \\

\bottomrule
\end{tabular}
}
\label{tab:mos_result}
\end{table}

==> tables/mos_table_backup.tex <==
\begin{table}
\caption{Objective (MCD in dB, lower is better) and subjective (MOS, higher is better) naturalness evaluation results. The columns contain the identifier and type of the speaker (healthy/oral cancer).  (\textdagger) indicat ation is statistically significant at $p < 0.05$. (*) in the case of the MOS indicates that the reduction in MOS is statistically significant at $p < 0.05$. Gender: m stands for male, while f stands for female.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc|ccccc}
\toprule
 {} & \multicolumn{2}{|c|}{Healthy} & \multicolumn{5}{|c}{Oral cancer}  \\
 \midrule
{ID} & 01 & 07 & 02 &   03 &   04 & 05 & 06 \\
\midrule
Gender & m & f & m & m & m & f & f \\
\midrule
\multicolumn{8}{c}{SYNTHESIS} \\
\midrule
MCD & 7.91 & 8.67(\textdagger) & 8.16 & 8.88(\textdagger) & 7.16(\textdagger) & 8.31(\textdagger) & 8.48 (\textdagger) \\
%$\emptyset$ &   7.48  &   7.59  &   7.09  &     8.38  &     6.65  &   7.79  &   7.34 \\
%.001    &   7.48  &   7.59  &   7.08  &     8.38  &     6.62  &   7.79  &   7.35 \\
%.01     &   7.41  &   7.57  &   7.08  &  8.06 (*) &     6.61  &   7.66  &   7.25 \\
%.1      &   7.36  &    7.5  &   7.05  &     8.46  &  6.58 (*) &   8.02  &    7.3  \\
\midrule
ground truth MOS    &     4.73 &     4.89 &     3.96 &     4.02 &     3.37 &     4.33 &     4.17 \\
resynthesis MOS &     4.13 (*) &     4.73 (*) &     3.49 (*) &     3.39 (*) &     3.24 &     3.93 (*)  &     4.03 \\
predicted MOS   &     2.28 (*) &     2.87 (*) &     2.19 (*) &     1.93 (*) &     2.23 (*) &     2.62 (*) &     2.26 (*) \\
\midrule
\multicolumn{8}{c}{MANIPULATION} \\
\midrule
MCD & 7.5(\textdagger) & 7.36(\textdagger) & 7.05(\textdagger) & 8.06(*) & 6.58 (*) & 7.79 & 7.3(\textdagger) \\ 
\bottomrule

\end{tabular}

\label{tab:mcd_result}
}
\vspace{-2 em}
\end{table}

